Impacts of floating-point non-associativity on reproducibility for HPC and deep learning applications

Run to run variability in parallel programs caused by floating-point non-associativity has been known to significantly affect reproducibility in iterative algorithms, due to accumulating errors. Non-reproducibility can critically affect the efficiency and effectiveness of correctness testing for stochastic programs. Recently, the sensitivity of deep learning training and inference pipelines to floating-point non-associativity has been found to sometimes be extreme. It can prevent certification for commercial applications, accurate assessment of robustness and sensitivity, and bug detection. New approaches in scientific computing applications have coupled deep learning models with high-performance computing, leading to an aggravation of debugging and testing challenges. Here we perform an investigation of the statistical properties of floating-point non-associativity within modern parallel programming models, and analyze performance and productivity impacts of replacing atomic operations with deterministic alternatives on GPUs. We examine the recently-added deterministic options in PyTorch within the context of GPU deployment for deep learning, uncovering and quantifying the impacts of input parameters triggering run to run variability and reporting on the reliability and completeness of the documentation. Finally, we evaluate the strategy of exploiting automatic determinism that could be provided by deterministic hardware, using the Groq accelerator for inference portions of the deep learning pipeline. We demonstrate the benefits that a hardware-based strategy can provide within reproducibility and correctness efforts.

==> Notes_etc/old_pytorch_sources_nd.tex <==
\subsection{Sources of non-determinism}
\comm{CC: maybe this subsection should be 1-2 paragraphs due to document length...}
In PyTorch, there are multiple potential sources of non-determinism, in particular:

\begin{itemize}
    \item{Unfixed RNG seed}
    \item{Unfixed CUDA environment variables}
    \item{Different algorithms being chosen at runtime, in particular cuDNN convolutions}
    \item{Non-deterministic memory initialization}
    \item{Non-existing deterministic algorithm implementations}
\end{itemize}

\com{CC: I think we should get rid of the torch.module.blah in some cases, users will have to refer to documentation}

In PyTorch, the RNG seed for both CUDA and CPU tensors can be fixed via the \texttt{torch.manual\_seed()} API call. In particular, setting this RNG seed will ensure all initialised torch tensors, including model weights to be run by run deterministic. Non-determinism can also be introduced via the Torch DataLoader which will reseed workers by default. Fix the worker seed via the \texttt{worker\_init\_fn()} API call and fix the \texttt{torch.Generator()} generator RNG seed to ensure reproducibility. Caution must be exercised to ensure any RNG seeds introduced via other frameworks are fixed. For example, a user casting a NumPy ndarray to a Torch tensor must ensure the global NumPy RNG seed is fixed via the \texttt{numpy.random.seed()} API call. A user using custom torch operators must fix the global python seed via the \texttt{random.seed()} API call.

According to the NVIDIA cuBLAS documentation, determinism is guaranteed for cuBLAS API calls from the same toolkit version for GPUs with identical architecture and identical number of Streaming MultiProcessors.
Determinism holds for a single CUDA stream. Multiple streams may lead to non-deterministic introduced due to optimization. To ensure determinism with multiple streams, a user may set a debug environment variable \texttt{CUBLAS\_WORKSPACE\_CONFIG}. There are two choices of environment variable, \texttt{:16:8} will limit performance while \texttt{:4096:8} increases GPU memory footprint. 

CUDA convolution operations call the cuDNN library. The cuDNN library may introduce nondeterminism via its benchmarking feature. This runtime benchmark feature selects the most performant algorithm based on the hyperparamters. This selection may vary run to run due to hardware differences and random benchmarking noise. Benchmarking can be disabled via  \texttt{torch.backends.cudnn.benchmark = False} . This will ensure a fixed convolution algorithm selection, potentially at the expense of performance. Note, the fixed convolution algorithm itself may not be run-by-run deterministic.

Initialization operations including \texttt{torch.empty()} and \texttt{torch.Tensor.resize\_()} may create tensors with uninitialized memory, leading to nondeterministic  downstream results.A user can set uninitialized memory with known values by setting the \texttt{torch.utils.deterministic.fill\_uninitialized\_memory} flag to True This will ensure determinism, with a potential performance penalty. If your program doesn't use uninitialized memory, you can disable this setting for better performance. Note the \texttt{torch.use\_deterministic\_algorithm} flag has to be set to True in addition to the \texttt{torch.utils.deterministic.fill\_uninitialized\_memory} flag

The \texttt{torch.use\_deterministic\_algorithms()} API call configures PyTorch to use deterministic algorithms instead of nondeterministic ones where available, and to throw a \texttt{RuntimeError} if an operation is known to be nondeterministic, without a deterministic implementation. To reiterate, there are two classes of non-deterministic operations.

\begin{itemize}
    \item{Non-deterministic operations with deterministic implementations, and}
    \item{Non-deterministic operations without deterministic implementations}
\end{itemize}

An exhausitve list of operations from each set can be found in the torch documentation \cite{https://pytorch.org/docs/stable/generated/torch.use_deterministic_algorithms.html} In general, the operations are either a convolution, scatter, gather or padding operation or involve sorting and/or summing values across tensors. Each of these operations in turn have various hyperparameters, some of which are only determined at runtime. Some operations are specified in the documentation \cite{https://pytorch.org/docs/stable/generated/torch.use_deterministic_algorithms.html} to be non-deterministic only under certain conditions. For example, \texttt{torch.Tensor.scatter\_reduce()} when reduce='sum' or reduce='mean' and called on CUDA tensor and torch.nn.MaxPool3d when attempting to differentiate a CUDA tensor. We have noticed that eventhough the documentation states torch.NLLLoss does not have a deterministic implementation, and should throw a RuntimeError when torch.use\_deterministic\_algorithms = True, the operation runs, and looks to run deterministically. This motivates a study of the non-deterministic ops and the regimes in which non-determinism appear. In particular, we investigate:

\begin{itemize}
    \item {The set of hyperparameters for each operation which exhibits non-determinism, and the severity of this non-determinism. We note the metrics used in more detail in the following section.}
    \item{Trends for non-determinism, i.e does increasing the kernel size of a Conv2d layer increase the severity of non-determinism?}
    \item{The latency difference between deterministic and non-deterministic implementation of the same algorithm. We would like to understand if performance loss is always incurred when using a deterministic implementation, and to what extent.}
    \item{Explore novel architectures, in particular The Groq LPU as an alternative platform which is deterministic by default. Note the Groq LPU is inference focued, and therefore kernels which are non-deterministic in the backward call are not investigated on Groq.}
\end{itemize} 
